GK Per 2015 dwarf nova covered by Suzaku

The intermediate polar GK Per exhibited a dwarf nova outburst in March-April 2015. Suzaku X-ray telescope serendipitously captured the onset of the outburst during its pre-scheduled pointing observation spanning four days. In this paper, we present temporal and spectral analysis results of this outburst, together with those from archival data of quiescent obtained in 2009 and 2014. Our temporal analysis confirmed previously reported spin modulation of X-ray count rates in outburst with a WD spin period of P_WD=351.4+/-0.5 s. The modulation is also detected in the hard X-ray band (16-60 keV), and spectral modeling of the absorption suggests obscuration by a dense absorption with a line-of-sight column density of N_H>10^23 cm^-2. A complex time evolution of spin modulation profiles is seen; the spin minimum phase shifts from phase ~0.25 in the first half of the observation to ~0.65 in the second one, and the pulse shape significantly changes epoch by epoch. Spectral fitting in the Fe Kalpha band revealed an increase of the fluorescent line equivalent width, from ~80 eV (quiescent) to ~140 eV (outburst). The equivalent widths of He-like and H-like Fe Kalpha are consistent with being constant at ~40 eV in the two states. Broad-band spectral fitting in the 2-60 keV band resulted in a sub-solar Fe abundance of ~0.1 Z_sun and the maximum plasma temperature kT_max~50-60 keV when the isobaric cooling flow model was applied. Based on the very small temperature change against a 6-7-times increased accretion rate, the accretion geometry in early outburst is discussed.

==> figures/Makefile <==
ANALYSIS_ROOT = $(HOME)/work/suzaku/gkper
DIR_PLOTS = $(ANALYSIS_ROOT)/plots/lc_xis

all: swiftLC.pdf \
 fi_evt_source_ra_dec_120_1st.pdf \
 fi_evt_source_ra_dec_120_2nd.pdf \
 fi_evt_source_ra_dec_120_3rd.pdf \
 hxd_lightcurve.pdf \
 hxd_fit_brems.pdf \
 hxd_fit_pow_brems.pdf \
 xis_123.pdf \
 xis_123_match7_10keV.pdf \
 xis_3rd_spectra_all_intervals.pdf \
 xis_3rd_spectra_all_intervals_scaled.pdf \
 fe_line.pdf \
 folded_lc_soft.pdf \
 folded_lc_mid.pdf \
 folded_lc_hard.pdf \
 folded_lc_all_16_60.pdf \
 nH_vs_FeI_EW.pdf \
 broad_band_fit.pdf
  
#---------------------------------------------
../../swift/SwiftBAT-Suzaku.pdf: ../../swift/GKPer.lc.txt ../../swift/go_plot.sh
	make -C ../../swift

swiftLC.pdf: ../../swift/SwiftBAT-Suzaku.pdf
	make -C ../../swift
	cp $^ $@

#---------------------------------------------
fi_evt_source_ra_dec_120_1st.pdf: $(DIR_PLOTS)/fi_evt_source_ra_dec_120_1st.pdf
	cp $^ $@
fi_evt_source_ra_dec_120_2nd.pdf: $(DIR_PLOTS)/fi_evt_source_ra_dec_120_2nd.pdf
	cp $^ $@
fi_evt_source_ra_dec_120_3rd.pdf: $(DIR_PLOTS)/fi_evt_source_ra_dec_120_3rd.pdf
	cp $^ $@

#---------------------------------------------
hxd_lightcurve.pdf: $(ANALYSIS_ROOT)/3rd/analysis/pin/lightcurve_analysis/plots/hardnessratio/hardnessratio.pdf
	cp $^ $@

#---------------------------------------------
hxd_fit_brems.pdf: $(ANALYSIS_ROOT)/409018020/analysis/pin/spectral_analysis/fittings/intervals_brems.pdf
	cp $^ $@

#---------------------------------------------
hxd_fit_pow_brems.pdf: $(ANALYSIS_ROOT)/409018020/analysis/pin/spectral_analysis/fittings/intervals_PhoIndex_kT.pdf
	cp $^ $@

#---------------------------------------------
xis_123.pdf: $(ANALYSIS_ROOT)/plots/spec_xis_for_paper/xis_123.pdf
	cp $^ $@

xis_123_match7_10keV.pdf: $(ANALYSIS_ROOT)/plots/spec_xis_for_paper/xis_123_match7_10keV.pdf
	cp $^ $@

#---------------------------------------------
xis_3rd_spectra_all_intervals.pdf: $(ANALYSIS_ROOT)/409018020/analysis/xis/spectral_analysis/plots/spectra_intervals.pdf
	cp $^ $@

#---------------------------------------------
xis_3rd_spectra_all_intervals_scaled.pdf: $(ANALYSIS_ROOT)/409018020/analysis/xis/spectral_analysis/plots/spectra_intervals_scaled.pdf
	cp $^ $@

#---------------------------------------------
fe_line.pdf: $(ANALYSIS_ROOT)/plots/fe_line/fe_line.pdf
	cp $^ $@

#---------------------------------------------
folded_lc_soft.pdf: $(ANALYSIS_ROOT)/409018020/analysis/xis/lightcurve_analysis/efold_root/folded_lc_soft.pdf
	cp $^ $@
folded_lc_hard.pdf: $(ANALYSIS_ROOT)/409018020/analysis/xis/lightcurve_analysis/efold_root/folded_lc_hard.pdf
	cp $^ $@
folded_lc_all_16_60.pdf: $(ANALYSIS_ROOT)/409018020/analysis/pin/lightcurve_analysis/efold_root/folded_lc_all_16_60.pdf
	cp $^ $@

#---------------------------------------------
nH_vs_FeI_EW.pdf: $(ANALYSIS_ROOT)/plots/nH_vs_feLine/nH_vs_FeI_EW.pdf 
	cp $^ $@

#---------------------------------------------
broad_band_fit.pdf: $(ANALYSIS_ROOT)/plots/plot_phabs_pcfabs_reflect_mkcflow_gaus/broad_band_fit.pdf
	cp $^ $@

==> tables/Makefile <==
ANALYSIS_ROOT = $(HOME)/work/suzaku/gkper

all: \
	table_hxd_pow_brems.tex fe_line.tex \
	folded_lc_table.tex \
	table_phabs_brems_phabs_brems.tex \
	table_phabs_pcfabs_reflect_mkcflow_gaus.tex

table_hxd_pow_brems.tex: $(ANALYSIS_ROOT)/409018020/analysis/pin/spectral_analysis/fittings/table_hxd_pow_brems.tex
	cp $^ $@

fe_line.tex : $(ANALYSIS_ROOT)/plots/fe_line/fe_line.tex
	cp $^ $@

folded_lc_table.tex: $(ANALYSIS_ROOT)/409018020/analysis/xis/lightcurve_analysis/efold_root/folded_lc_table.tex
	cp $^ $@

table_phabs_brems_phabs_brems.tex: $(ANALYSIS_ROOT)/409018020/analysis/xis/spectral_analysis/fittings/table_phabs_brems_phabs_brems.tex
	cp $^ $@

table_phabs_pcfabs_reflect_mkcflow_gaus.tex: $(ANALYSIS_ROOT)/409018020/analysis/simultaneous/table/table_fit_phabs_pcfabs_reflect_mkcflow_gaus.tex
	cp $^ $@


==> tables/table_phabs_pcfabs_reflect_mkcflow_gaus.tex <==
\hline
Epoch & $N_{\mathrm{H}}$   & $N_{\mathrm{H}}$ & C.F. & Highest $kT$ & $Z_{\mathrm{Fe}}$ & $\chi^2/\nu~(\nu)$\\
      & $10^{22}$~cm$^{-2}$ & $10^{22}$~cm$^{-2}$ &      & keV          & $Z_\odot$          & \\
\hline
0 & $1.79^{+0.16}_{-0.09}$ & $62.2^{+31.5}_{-47.9}$ & $0.17^{+0.17}_{-0.15}$ & $41.8^{+9.8}_{-9.8}$ & $0.10^{+0.06}_{-0.05}$ & $0.94$ (1308)\\
1 & $2.60^{+0.13}_{-0.15}$ & $64.3^{+15.9}_{-20.1}$ & $0.30^{+0.09}_{-0.10}$ & $45.1^{+8.6}_{-6.8}$ & $0.09^{+0.04}_{-0.03}$ & $1.04$ (1782)\\
2 & $3.53^{+0.22}_{-0.29}$ & $23.6^{+8.3}_{-6.7}$ & $0.35^{+0.03}_{-0.03}$ & $59.3^{+4.7}_{-5.0}$ & $0.12^{+0.03}_{-0.02}$ & $0.99$ (1980)\\
3 & $3.75^{+0.16}_{-0.17}$ & $40.7^{+7.4}_{-6.8}$ & $0.45^{+0.03}_{-0.03}$ & $55.2^{+5.1}_{-5.0}$ & $0.08^{+0.02}_{-0.02}$ & $1.06$ (2007)\\
4 & $5.50^{+0.22}_{-0.23}$ & $41.2^{+7.6}_{-6.8}$ & $0.49^{+0.03}_{-0.02}$ & $59.4^{+5.9}_{-5.7}$ & $0.10^{+0.02}_{-0.02}$ & $1.03$ (2011)\\
5 & $4.88^{+0.23}_{-0.23}$ & $34.6^{+5.9}_{-4.9}$ & $0.53^{+0.02}_{-0.02}$ & $59.7^{+4.6}_{-4.8}$ & $0.11^{+0.02}_{-0.02}$ & $1.10$ (2056)\\
\hline\\
